Large-scale magnetic field maps using structured kernel interpolation for Gaussian process regression

We present a mapping algorithm to compute large-scale magnetic field maps in indoor environments with approximate Gaussian process (GP) regression. Mapping the spatial variations in the ambient magnetic field can be used for localization algorithms in indoor areas. To compute such a map, GP regression is a suitable tool because it provides predictions of the magnetic field at new locations along with uncertainty quantification. Because full GP regression has a complexity that grows cubically with the number of data points, approximations for GPs have been extensively studied. In this paper, we build on the structured kernel interpolation (SKI) framework, speeding up inference by exploiting efficient Krylov subspace methods. More specifically, we incorporate SKI with derivatives (D-SKI) into the scalar potential model for magnetic field modeling and compute both predictive mean and covariance with a complexity that is linear in the data points. In our simulations, we show that our method achieves better accuracy than current state-of-the-art methods on magnetic field maps with a growing mapping area. In our large-scale experiments, we construct magnetic field maps from up to 40000 three-dimensional magnetic field measurements in less than two minutes on a standard laptop.

==> 0_Parking.tex <==
This elementwise computation for the linear kernel leads to the $3 \times 3$ diagonal kernel function $\kappab_{\crm}(\pb,\pb')$, describing the constant deviations of Earth's magnetic field.
For the squared exponential kernel, this leads to a curl-free extension of the squared exponential kernel capable of learning curl-free vector fields~\cite{wahlstrom2015modeling}.
This kernel function is given by
\begin{equation}
    \label{eq:covcurl}
    \kappab(\pb,\pb') = \frac{\sfac^2}{\ell^2} \exp\left(-\frac{||\pb-\pb'||^2}{2\ell^2} \right) \left(\Ib_3 - \left(\frac{\pb-\pb'}{\ell}\right)\left(\cdot\right)^\top\right).
\end{equation}
Using the derived $3 \times 3$ kernel functions $\kappab_{\crm}(\pb,\pb')$ and $\kappab_{\SE}(\pb,\pb')$, the scalar potential model can equivalently be written as a multi-output Gaussian process model~\cite{wahlstrom2015modeling}, given by
\begin{equation}
    \label{eq:curlmodel}
    \begin{aligned}
    \Hb(\pb) &\sim \mathcal{GP}\left(\zerob,\kappab_{\crm}(\pb,\pb') + \kappab(\pb,\pb')\right),\\
    \yb_n &= \Hb(\pb_n) + \eb_n, \hspace{5mm} \eb_n \sim \N(\zerob, \sn^2 \Ib_3),
    \end{aligned}
\end{equation}
